Centered colorings and weak coloring numbers in minor-closed graph classes

Let $\mathcal{C}$ be a proper minor-closed class of graphs. Given the minors excluded in $\mathcal{C}$, we determine the maximum $q$-centered chromatic number and the maximum $q$th weak coloring number of graphs in $\mathcal{C}$ within an $\mathcal{O}(q)$-factor. Moreover, when $\mathcal{C}$ excludes a planar graph, we determine it within a constant factor. Our results imply that the $q$-centered chromatic number of $K_t$-minor-free graphs is in $\mathcal{O}(q^{t-1})$, improving on the previously known $\mathcal{O}(q^{h(t)})$ bound with a large and non-explicit function $h$. We include similar bounds for another family of parameters, the fractional treedepth fragility rates. All our bounds are proved via the same general framework.

==> style.toc.tex <==
% https://tex.stackexchange.com/questions/633286/how-to-add-dots-to-ams-table-of-contents
\usepackage{xpatch}
\makeatletter   
\xpatchcmd{\@tocline}
{\hfil\hbox to\@pnumwidth{\@tocpagenum{#7}}\par}
{\ifnum#1<2\hfill\else\dotfill\fi\hbox to\@pnumwidth{\@tocpagenum{#7}}\par}
{}{}
\makeatother    
% *******************************************   

\makeatletter
\def\l@section{\bfseries\@tocline{1}{0pt}{0pc}{4pc}{}}
\def\l@subsection{\mdseries\@tocline{2}{0pt}{4pc}{6pc}{}}
%\def\l@subsubsection{\mdseries\@tocline{3}{0pt}{8pc}{8pc}{}}

% \renewcommand*\l@section[2]{%
%   \addvspace{0.15em}% <-- uniform vertical spacing
%   \bfseries
%   \@tocline{1}{0pt}{0pc}{4pc}{}{#1}{#2}%
% }

% \renewcommand*\l@subsection[2]{%
%   \addvspace{0.05em}% optional smaller spacing
%   \mdseries
%   \@tocline{2}{0pt}{4pc}{6pc}{}{#1}{#2}%
% }

\makeatother

\renewcommand\contentsname{\vspace{-1cm}}

